Confinement Control of Double Integrators using Partially Periodic Leader Trajectories

We consider a multi-agent confinement control problem in which a single leader has a purely repulsive effect on follower agents with double-integrator dynamics. By decomposing the leader's control inputs into periodic and aperiodic components, we show that the leader can be driven so as to guarantee confinement of the followers about a time-dependent trajectory in the plane. We use tools from averaging theory and an input-to-state stability type argument to derive conditions on the model parameters that guarantee confinement of the followers about the trajectory. For the case of a single follower, we show that if the follower starts at the origin, then the error in trajectory tracking can be made arbitrarily small depending on the frequency of the periodic control components and the rate of change of the trajectory. We validate our approach using simulations and experiments with a small mobile robot.

==> _preamble_hyperref.tex <==
%%fakepart{Setup autoreferencing}
%----------------------------------------------------------------------|

\usepackage{varioref}
\labelformat{subfigure}{\thefigure\textup{(#1)}}
\labelformat{equation}{\textup{(#1)}}
%\labelformat{enumi}{\textup{(#1)}}

% Hyperref is not just about links...
\RequirePackage[svgnames]{xcolor}
\usepackage[%
        pagebackref=false,
        bookmarks=true,bookmarksopen=true,
        bookmarksnumbered=true,
        breaklinks=true,
        colorlinks=true,
        anchorcolor=blue,citecolor=blue,
        urlcolor=blue,linkcolor=blue,filecolor=blue,
        menucolor=blue,
        %pdfpagelabels=true,hypertexnames=false,
        %plainpages=false,
    ]{hyperref}
\usepackage{url}
\urlstyle{same}
% Gives us a \url that breaks
%\usepackage{breakurl}
% Give us a \doi that links
\usepackage{doi}
\def\doitext{doi:~}
\newcommand\emaillink[1]{\href{mailto:#1}{#1}}

% Prefer to use package subfig instead, but use old subfigure for
% technical reasons.
\usepackage{subfigure}

% Fixes a problem with how old versions of hyperref record item labels
\makeatletter
\@ifpackageloaded{hyperref}{%
\@ifpackageloaded{amsmath}{%
\newcommand{\AMShreffix}[1]{%
        \expandafter\let\csname AMShreffix#1\expandafter\endcsname%
                \csname #1\endcsname%
        \expandafter\renewcommand\csname #1\endcsname{%
                \@hyper@itemfalse\csname AMShreffix#1\endcsname}}
\AtBeginDocument{%
\AMShreffix{equation}
\AMShreffix{align}
\AMShreffix{alignat}
\AMShreffix{flalign}
\AMShreffix{gather}
\AMShreffix{multline}
}}{}}{}
\makeatother

% Need to redefine \autoref. Should use abbreviations inside the
% sentence and full names at the beginning of sentences. Additionally,
% need to handle the plural cases.

\def\subfigureautorefname{\figureautorefname}
\def\subfloatautorefname{\figureautorefname}
%
\def\subsectionautorefname{\sectionautorefname}
\def\subsubsectionautorefname{\sectionautorefname}
%
\def\subappendixautorefname{\appendixautorefname}
\def\subsubappendixautorefname{\appendixautorefname}
\def\appendixparagraphautorefname{\appendixautorefname}

% % Use Fig.
\def\figurename{Fig.}
% Use Figure
%\def\figurename{Figure}

% \Autoref is for the beginning of the sentence
\let\orgautoref\autoref
\providecommand{\Autoref}
        {\def\equationautorefname{Equation}%
         \def\figureautorefname{Figure}%
         \def\sectionautorefname{Section}%
         \def\subsectionautorefname{\sectionautorefname}%
         \def\appendixautorefname{Appendix}%
         \def\Itemautorefname{Item}%
         \def\tableautorefname{Table}%
         \def\thmautorefname{Theorem}%
         \def\lemautorefname{Lemma}%
         \def\propautorefname{Proposition}%
         \def\asmpautorefname{Assumption}%
         \def\corautorefname{Corollary}%
         \def\defnautorefname{Definition}%
         \def\conjautorefname{Conjecture}%
         \def\exmpautorefname{Example}%
         \def\remautorefname{Remark}%
         \def\noteautorefname{Note}%
         \def\caseautorefname{Case}%
         \orgautoref}

% \Autorefs is plural for the beginning of the sentence
\providecommand{\Autorefs}
        {\def\equationautorefname{Equations}%
         \def\figureautorefname{Figures}%
         \def\sectionautorefname{Sections}%
         \def\subsectionautorefname{\sectionautorefname}%
         \def\appendixautorefname{Appendices}%
         \def\Itemautorefname{Items}%
         \def\tableautorefname{Tables}%
         \def\thmautorefname{Theorems}%
         \def\lemautorefname{Lemmas}%
         \def\propautorefname{Propositions}%
         \def\asmpautorefname{Assumptions}%
         \def\corautorefname{Corollaries}%
         \def\defnautorefname{Definitions}%
         \def\conjautorefname{Conjectures}%
         \def\exmpautorefname{Examples}%
         \def\remautorefname{Remarks}%
         \def\noteautorefname{Notes}%
         \def\caseautorefname{Cases}%
         \orgautoref}

% Get rid of space (if desired)
\def\Enospace~{}

% \autoref is used inside a sentence (renew of the standard autoref)
\renewcommand{\autoref}
        {\def\equationautorefname{Eq.}%
         \def\figureautorefname{Fig.}%
         \def\sectionautorefname{Sect.}%
         \def\subsectionautorefname{\sectionautorefname}%
         \def\appendixautorefname{Appendix}%
         \def\Itemautorefname{item}%
         \def\tableautorefname{Table}%
         \def\thmautorefname{Theorem}%
         \def\lemautorefname{Lemma}%
         \def\propautorefname{Proposition}%
         \def\asmpautorefname{Assumption}%
         \def\corautorefname{Corollary}%
         \def\defnautorefname{Definition}%
         \def\conjautorefname{Conjecture}%
         \def\exmpautorefname{Example}%
         \def\remautorefname{Remark}%
         \def\noteautorefname{Note}%
         \def\caseautorefname{Case}%
         \orgautoref}

% \autorefs is plural for inside a sentence
\providecommand{\autorefs}
        {\def\equationautorefname{Eqs.}%
         \def\figureautorefname{Figs.}%
         \def\sectionautorefname{Sects.}%
         \def\subsectionautorefname{\sectionautorefname}%
         \def\appendixautorefname{Appendices}%
         \def\Itemautorefname{items}%
         \def\tableautorefname{Tables}%
         \def\thmautorefname{Theorems}%
         \def\lemautorefname{Lemmas}%
         \def\propautorefname{Propositions}%
         \def\asmpautorefname{Assumptions}%
         \def\corautorefname{Corollaries}%
         \def\defnautorefname{Definitions}%
         \def\conjautorefname{Conjectures}%
         \def\exmpautorefname{Examples}%
         \def\remautorefname{Remarks}%
         \def\noteautorefname{Notes}%
         \def\caseautorefname{Cases}%
         \orgautoref}

% Make \title integrate PDF title and bookmark and build \thetitle
% \let\oldtitle\title
% \renewcommand\title[1]{%
%     \begingroup
%         \hypersetup{pdftitle={#1}}%
%         \def\thetitle{#1}%
%         \pdfbookmark[0]{#1}{title}
%     \endgroup
%     \oldtitle{#1}%
% }
%
% % Give us a \mykeywords
% \newcommand\mykeywords[1]{%
%     \begingroup
%         \providecommand{\and}{}%
%         \renewcommand{\and}{\unskip, }%
%         \hypersetup{pdfkeywords={#1}}%
%         \xdef\thekeywords{#1.}%
%     \endgroup}
%
% % Give us a \myauthors
% \newcommand\myauthors[1]{%
%     \begingroup
%         \providecommand{\and}{}%
%         \renewcommand{\and}{\unskip, }%
%         \hypersetup{pdfauthor={#1}}%
%         \xdef\theauthors{#1}%
%     \endgroup}

%----------------------------------------------------------------------|

%%fakepart{Setup indexing}
%----------------------------------------------------------------------|

% \usepackage{makeidx}
% \makeindex             % used for the subject index
%                        % please use the style svind.ist with
%                        % your makeindex program

%----------------------------------------------------------------------|

